Individually-Fair Auctions for Multi-Slot Sponsored Search

We design fair sponsored search auctions that achieve a near-optimal tradeoff between fairness and quality. Our work builds upon the model and auction design of Chawla and Jagadeesan \cite{CJ22}, who considered the special case of a single slot. We consider sponsored search settings with multiple slots and the standard model of click through rates that are multiplicatively separable into an advertiser-specific component and a slot-specific component. When similar users have similar advertiser-specific click through rates, our auctions achieve the same near-optimal tradeoff between fairness and quality as in \cite{CJ22}. When similar users can have different advertiser-specific preferences, we show that a preference-based fairness guarantee holds. Finally, we provide a computationally efficient algorithm for computing payments for our auctions as well as those in previous work, resolving another open direction from \cite{CJ22}.

==> PA/posAuc.tex <==
In the case of \kipaname, we had to remove advertisers with unallocated amounts greater than $1$ before giving the remaining advertisers their assignments. Similarly, for \kpaname, we start by finding the advertisers whose proportional allocation would be more than $1$, instead assigning them an allocation of exactly $1$ and removing them from consideration. Then, we allocate the remaining mass proportionally among the remaining advertisers. Note that this step is unnecessary in the $1$-unit case, so setting $k=1$ means that the while loop never executes and the mechanism reduces to that presented in \cite{CIJ20_Multi_Category_Fairness}.

\vspace{0.5 cm}
\begin{algorithm}[H]
 \textbf{Input: }Vector $v$ of non-negative advertiser bids for user $u$; ad-specific CTRs $\userCTR_1, \cdots, \userCTR_n$; number of slots $\numberOfSlots$; a continuous, increasing, super-additive function $g:\mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^{\geq 0}$\;
 \textbf{Initialization: }
 Determine effective values, $\effv_i=v_i\alpha_i$ for all $i$\;
 WLOG assume $\effv_1 \geq \ldots\geq \effv_{\numberOfAdvertisers}$\;
 Set $s \leftarrow 1$\;
 Set $h \leftarrow \numberOfAdvertisers$\;
 \While{$\frac {h\cdot{} g(\effv_s)}{\sum_{t=s}^{n} g(\effv_t) } > 1$}{
  $\kpa_s\leftarrow 1$\;
  $s\leftarrow s+1$\;
  $h\leftarrow h-1$\;}
  For $i\geq s$ set $\kpa_i \leftarrow \frac {h\cdot{} g(\effv_1) }{ \sum_{t=s}^{n} g(\effv_t) }$\;
  \Return $\kpa$
 \caption{\kpaname}\label{alg:k-unit-PA}
\end{algorithm}
\vspace{0.5 cm}

Next, we extend the \kpaname\ to the \separablesetting\ in the same manner we extended \kipaname. We call this algorithm \mpaname. 
For every slot $j$, the distribution over advertisers is given by the difference between the $j$-unit and $j-1$-unit allocations produced by \kpaname.

\vspace{0.5 cm}
\begin{algorithm}[H]
 \textbf{Input: }Vector $v$ of non-negative advertiser bids for user $u$; CTRs $\userCTR_1, \cdots, \userCTR_n$ and $\slotCTR_1, \cdots, \slotCTR_{\numberOfSlots}$; number of slots $\numberOfSlots$; a continuous, increasing, super-additive function $g:\mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^{\geq 0}$\;
 \textbf{Initialization: }WLOG assume $\alpha_1v_1\geq \ldots\geq \alpha_{\numberOfAdvertisers}v_{\numberOfAdvertisers}$\;
 \For {$h \in [k]$}{Set $\kpah{h}\leftarrow$ the output of \kpaname\ on input $(v, \userCTRVector, h, g)$}
 \For{$j \in [\numberOfSlots]$}{Set $\mpa_{\cdot,j} = \kpah{j} - \kpah{j-1}$ }
 \Return \mpa
 \caption{\mpaname}\label{alg:PA-General}
\end{algorithm}
\vspace{0.5 cm}

Note that, like \Cref{alg:IPA-separable}, \Cref{alg:PA-General} is scale-free and independent of $\beta$. It also has the same property on the marginal row sums-- for every advertiser $i$, the sum of the allocation to the first $j$ slots is equal to the $j$-unit allocation to advertiser $i$. This allows us to extend the social welfare guarantees from \originalpaname\ to the \separablesetting\ while maintaining an appropriate generalization of the value stability condition, as we formally prove in the rest of this section.

